What is the Role of Large Language Models in the Evolution of Astronomy Research?

ChatGPT and other state-of-the-art large language models (LLMs) are rapidly transforming multiple fields, offering powerful tools for a wide range of applications. These models, commonly trained on vast datasets, exhibit human-like text generation capabilities, making them useful for research tasks such as ideation, literature review, coding, drafting, and outreach. We conducted a study involving 13 astronomers at different career stages and research fields to explore LLM applications across diverse tasks over several months and to evaluate their performance in research-related activities. This work was accompanied by an anonymous survey assessing participants' experiences and attitudes towards LLMs. We provide a detailed analysis of the tasks attempted and the survey answers, along with specific output examples. Our findings highlight both the potential and limitations of LLMs in supporting research while also addressing general and research-specific ethical considerations. We conclude with a series of recommendations, emphasizing the need for researchers to complement LLMs with critical thinking and domain expertise, ensuring these tools serve as aids rather than substitutes for rigorous scientific inquiry.

==> rasti_coverletter.tex <==
Dear Members of the Editorial Board,

I am writing to submit our manuscript, "The Role of Large Language Models in the Evolution of Astronomy Research: An Evaluation of Performance and Ethical Considerations," to the RASTI journal. 

This work investigates the transformative impact of large language models (LLMs) on astronomy, exploring their potential and limitations in research-related activities. We have confirmed with Jonathan Tennyson that this work is within the scope of the journal, ensuring its relevance to your readership. 

In our manuscript, we comprehensively evaluate LLMs and their effectiveness in enhancing various aspects of astronomy research. Through our analysis, we aim to illuminate the capabilities of these AI tools while also addressing the ethical considerations that arise with their use. We recognize that while LLMs can significantly advance research efficiency and data analysis, they are not without their challenges, including issues of bias, misinformation, and the risk of over-reliance on automated systems.
Our concluding recommendations emphasize the critical need for researchers to integrate LLMs with robust critical thinking and analytical skills. We believe that this complementary approach will enable astronomers to harness the full potential of AI while maintaining the integrity and rigor of the scientific process.

We are confident that our findings will contribute valuable insights to the ongoing discourse surrounding the integration of AI in scientific research. Given the RASTI journal's commitment to exploring innovative methodologies and technologies in research, we believe our manuscript aligns perfectly with your publication's objectives.
Thank you for considering our submission. We look forward to the opportunity to contribute to the RASTI journal and share our insights with the broader academic community.
Sincerely,
